Statistical solutions of hyperbolic systems of conservation laws: numerical approximation

Statistical solutions are time-parameterized probability measures on spaces of integrable functions, that have been proposed recently as a framework for global solutions and uncertainty quantification for multi-dimensional hyperbolic system of conservation laws. By combining high-resolution finite volume methods with a Monte Carlo sampling procedure, we present a numerical algorithm to approximate statistical solutions. Under verifiable assumptions on the finite volume method, we prove that the approximations, generated by the proposed algorithm, converge in an appropriate topology to a statistical solution. Numerical experiments illustrating the convergence theory and revealing interesting properties of statistical solutions, are also presented.

==> algorithm/fvm.tex <==
%!TEX root = ../main.tex

\subsection{Multidimensional Finite volume framework}

\label{sec:fvm}
This section briefly describes the conventional approach of numerically approximating conservation laws through finite volume and finite difference methods. For a complete review, one can consult~\cite{leveque_green}.

We discretize the computational spatial domain as a collection of cells
\[\big\{(x^1_{i_1-\hf}, x^1_{i_1+\hf})\times\cdots\times(x^d_{i^d-\hf}, x^d_{i^d+\hf})\big\}_{(i^1,\ldots,i^d)}\subset \D,\]
with corresponding cell midpoints
\[x_{i^1,\ldots, i^d}:=\left(\frac{x^1_{i_1+\hf}+x^1_{i_1-\hf}}{2},\ldots,\frac{x^d_{i_d+\hf}+x^d_{i_d-\hf}}{2}\right).\]
For simplicity, we assume that our mesh is equidistant, that is,
\[x^k_{i^k+\hf} - x^k_{i^k-\hf} \equiv \Dx \qquad \forall\ k=1,\dots,d\]
for some $\Dx>0$. We will describe the semi-discrete case. For each cell, marked by $(i^1,\ldots, i^d)$, we let $u^{\Dx}_{i^1,\ldots, i^d}(t)$ denote the averaged value in the cell at time $t\geq 0$.

We use the following semi-discrete formulation:
\begin{equation}\label{eq:semi_d}
\begin{split}
\ddt{}u^{\Dx}_{i^1,\ldots,i^d}(t)+\sum_{k=1}^d\frac{1}{\Dx}\left(F^{k,\Dx}_{i^1,\ldots,i^k+\hf,\ldots, i^d}(t)-F^{k,\Dx}_{i^1,\ldots,i^k-\hf,\ldots, i^d}(t)\right)= 0  \\
u^{\Dx}_{i^1,\ldots,i^d}(0) = u_0(x_{i^1,\ldots,i^d})
\end{split}
\end{equation}
where $F^{k,\Dx}$ is a \emph{numerical flux function} in direction $k$. In a \emph{$(2p+1)$-point scheme,} the numerical flux function $F^{k,\Dx}_{i^1,\ldots,i^k+hf,\ldots,i^d}(t)$ can be written as a function of $u^{\Dx}_{i^1,\ldots,j^k,\ldots,i^k}(t)$ for $j^k=i^k-p+1,\ldots,i^k+p$. We furthermore assume the numerical flux function is consistent with $f$ and locally Lipschitz continuous, which amounts to requiring that for every bounded set $K\subset \R$, there exists a constant $C>0$ such that for $k=1,\ldots,d$,
\begin{equation}
|F^{k,\Dx}_{i^1,\ldots,i^d}(t)-f(u^{\Dx}_{i^1,\ldots,i^d})|\leq C\sum_{j^k=i^1-p+1}^{i^k+p}|u^{\Dx}_{i^1,\ldots,i^d}(t)-u^{\Dx}_{i^1,\ldots, j^k,\ldots,i^d}(t)|,
\end{equation}
whenever $u^{\Dx}_{i^1,\ldots, i^k-p+1,\ldots,i^d}(t),\ldots, u^{\Dx}_{i^1,\ldots, i^k+p,\ldots, i^d}(t) \in K$.

We let
$\NumericalEvolution{\Dx}:L^\infty(\D)\to L^\infty(\DT)$
be the spatially discrete numerical evolution operator corresponding to \eqref{eq:semi_d}. Since $\NumericalEvolution{\Dx}$ is the composition of a projection from $L^\infty$ onto piecewise constant functions and a continuous evolution under an ordinary differential equation, we see that $\NumericalEvolution{\Dx}$ is measurable.

The current form of \eqref{eq:semi_d} is continuous in time, and one needs to employ a time stepping method to discretize the ODE in time, usually through some strong stability preserving Runge--Kutta method \cite{GST}.

Owing to $\NumericalEvolution{\Dx}$ being a measurable map, we can define an approximation of a statistical solution with initial data $\bar{\mu}$ as 
\begin{equation}
\label{eq:spatial_statistical}
\mu_t^{\Dx}=\pushforward{\NumericalEvolution{\Dx}(t)}{\bar{\mu}}.
\end{equation}


==> algorithm/mc.tex <==
%!TEX root = ../main.tex

\subsection{Monte Carlo algorithm}

While \eqref{eq:spatial_statistical} gives us an abstract definition of $\mu_t^{\Dx}$, it is not amenable for practical computations, since it requires the computation of the trajectory of almost all possible initial data $u_0\in\supp \bar{\mu}$. We thus turn to sampling algorithms.

The Monte Carlo algorithm has been shown to be robust in tackling high dimensional problems with low regularity~\cite{mlmc_hyperbolic,mlmc_hyperbolic-2}, and has later been demonstrated to perform well for measure valued solutions~\cite{fkmt}. For these reasons, we use the Monte Carlo algorithm. We use \Cref{alg:mc} to generate an approximation $\mu_t^{\Dx,M}$ of $\mu_t$. 


Using well known results for weak convergence of Monte Carlo\cite{vanderVaart1996}, we can conclude that we get a stochastic convergence rate of $1/2$. The following theorem makes this precise.

\todo[inline]{KOL: Do we want this convergence theorem here? Or move it to the section on convergence?}
\begin{theorem}
Let $\bar{\mu}\in \Prob(L^1(\D,\Ph))$ be the initial data, let $\NumericalEvolution{\Dx}$ be some numerical evolution operator, and let $\mu_t^{\Dx,M}$ be defined through \Cref{alg:mc} where $\Dx>0$ and $M\in\N$. Let $\mu_t^{\Dx}$ be defined by \eqref{eq:spatial_statistical}, then for every $g\in C_b(L^1(D))$, we have
\[\mathbb{E}((\Ypair{\mu_t^{\Dx,M}-\mu_t^{\Dx}}{g})^2)\leq \frac{\Var(\Ypair{\mu_t^{\Dx}}{g})}{M}.\]
\end{theorem}
Furthermore one can use the results \cite{wasserstein_mc_convergence} to get a convergence rate for the Wasserstein distance of the correlation marginals.\todo{KOL: Should this be included?}

\todo[inline]{KOL: Not sure if we should keep the algorithm environment, but it makes the disposition clean and readable, so I would be in favour of it.}
\begin{algorithm}[H]
 \KwData{initial $\bar{\mu}\in \Prob(L^1(\D,\Ph))$,
 	mesh width $\Dx>0$, numerical evolution operator $\NumericalEvolution{\Dx}$, number of samples $M\in\N$}
 Draw $M$ independent, identically distributed samples $\{u^k_0\}_{k=1}^M$ of $\bar{\mu}$\;
 \For{$k=1,\ldots, M$}{
  Evolve the sample in time $u_k^{\Dx}(t)=\NumericalEvolution{\Dx}(t)(u^k_0)$
 }
 Estimate statistical solution
 \begin{equation}
 \mu_t^{\Dx,M}:=\frac{1}{M}\sum_{k=1}^M \delta_{u_k(\omega; \cdot, t)},
 \end{equation}
 \caption{Monte Carlo algorithm for approximating statistical solutions.\label{alg:mc}}
\end{algorithm}

==> convergence/convergence.tex <==
    %!TEX root = ../main.tex
\section{Convergence of the algorithm to statistical solutions}
\input{convergence/compactness.tex}
\input{convergence/lax_wendroff.tex}


==> statistical_solutions/time_compactness.tex <==
%!TEX root = main.tex
\subsection{Time compactness of correlation measures}\label{sec:corrmeascompact} ~\\
\todo[inline]{Could still be typos!}
For a function $u\in L^p(D)$ we define the modulus of continuity
\begin{align*}
\omega_r^p(u) &:= \left(\int_D\intavg_{B_r(0)}|u(x+z)-u(x)|^p\,dzdx\right)^{1/p}.
\end{align*}
Throughout the text we will use the cutoff functions
\[
\theta(s) := \begin{cases}
1 & |s|\leq 1 \\
2-|s| & 1<|s|<2 \\
0 & |s|\geq2,
\end{cases}
\qquad \theta_M(v):=\theta(|v|/M),
\qquad \zeta_M(v) := v\theta_M(v)
\]
(for some $M>0$), defined for $s\in\R$ and $v\in\R^m$, where $m\in\N$ is an arbitrary integer. Note that $\zeta_M(v)=v$ for $|v|<M$ and $\zeta_M(v)=0$ for $|v|>2M$, and that $\|\zeta_M\|_{\Lip} \leq 2$.

\begin{lemma}\label{lem:cutoff}
If $u\in L^p(D,\R^m)$ then
\[
\big\|\zeta_M\circ u-u\big\|_{L^p(D)} \leq 3\omega_r^p(u)
\]
whenever $M \geq \frac{1}{|B_r|^{1/p}}\|u\|_{L^p(D)}$.
\end{lemma}
\begin{proof}
Denote $u_r(x) := \intavg_{B_r(0)}u(x+z)\,dz$. Then $|u_r(x)| \leq \frac{1}{|B_r|^{1/p}}\|u\|_{L^p(D)}$ for every $x\in D$, so that if $M \geq \frac{1}{|B_r|^{1/p}}\|u\|_{L^p(D)}$ then $u_r = \zeta_M\circ u_r$. It follows that
\begin{align*}
\big\|\zeta_M\circ u-u\big\|_{L^p(D)} &\leq \big\|\zeta_M\circ u-\zeta_M\circ u_r\big\|_{L^p(D)} + \|u_r-u\|_{L^p(D)} \\
&\leq \big(\|\zeta_M\|_{\rm Lip}+1\big)\|u_r-u\|_{L^p(D)} \\
&\leq 3\omega_r^p(u),
\end{align*}
where we have used the fact that $\|u_r-u\|_{L^p} \leq \omega_r^p(u)$.
\end{proof}

\todo[inline]{KOL: This theorem could probably be stated with $T=\infty$. Do we want this?}
\begin{theorem}\label{thm:trunccorrcompact}
Let $T>0$, and let $\cm_n \in L^p([0,T];\Corrmeas^{p}( D,U))$ for $n=1,2,\dots$ be a sequence of correlation measures such that
\begin{align}
\sup_{n\in\N}\int_0^T\Ypair{\nu^1_{t,n}}{|\xi|^p}_{\Caratheodory^1}\ dt &\leq c^p	\label{eq:uniformlpbound} \\
\lim_{r\to0}\sup_{n\in\N}\omega_r^p\bigl(\nu^2_{t,n}\bigr) &= 0 \qquad \text{for almost all }t\in [0,T)\label{eq:uniformdc}
\end{align}
for some $c>0$. Then there exists a subsequence $(n_j)_{j=1}^\infty$ and some $\cm\in L^p([0,T];\Corrmeas^{p}(D,U))$ such that 
\begin{enumerate}[label=\it (\roman*)]
\item $\int_0^T \Ypair{\nu_t^1}{|\xi|^p}_{\Caratheodory^1}\ dt \leq c^p$ 
\item $\cm_{n_j} \weaksto \cm$ as $j\to\infty$ 
\item for $k\in\N$, let $\phi\in L^1_{\textrm{loc}}(D^k)$, $\kappa\in C(U^k)$ and $\psi\in L^1([0,T])$ be nonnegative, and let $g(x,\xi) := \phi(x)\kappa(\xi)$. Then
\begin{equation}\label{eq:nuklimitbound}
\int_0^T\psi(t)\Ypair{\nu^k_t}{g}_{\Caratheodory^k}\dd t \leq \liminf_{j\to\infty} \int_0^T \psi(t)\Ypair{\nu_{t,n_j}^k}{g}_{\Caratheodory^k}\dd t.
\end{equation}

\item 

Assume moreover that 
\begin{align}
\limsup_{M\to\infty} \sup_{n\in\N} \int_0^T \int_{D\setminus B_M(0)} \Ypair{\nu^1_{n;x,t}}{|\xi|^p}\,dx dt &= 0, \label{eq:nutightness} \\
\|u\|_{L^p(D)} &\leq C \qquad \text{for $\mu_t$-a.e.\ } u\in L^p(D). \label{eq:LpLinftybound}
\end{align}
Then \emph{observables converge strongly:}
\begin{equation}\label{eq:nuklimit}
\lim_{j\to\infty}\int_{D^k} \big|\int_0^T\psi(t)\Ypair{\nu^k_{n_j,x,t}}{g(x)} - \psi(t)\Ypair{\nu^k_{x,t}}{g(x)}\ dt \big| \,dx= 0
\end{equation}
for any $\psi\in L^\infty([0,T])$, and for any Carath\'eodory function\footnote{A Carath\'eodory function is a function $g=g(x,\xi)$ such that $x\mapsto g(x,\xi)$ is measurable for all $\xi$ and $\xi\mapsto g(x,\xi)$ is continuous for almost every $x$.} $g:D^k\to C(U^k)$ satisfying both 
\begin{align*}
|g(x,\xi)|&\leq C_g\prod_{i=1}^k(1+|\xi_i|^p), \\
\big|g(x+z,\xi+\zeta)-g(x,\xi)\big| &\leq \kappa(z)|\zeta_i|\max\big(|\xi_i|,|\xi_i+\zeta_i|\big)^{p-1}\prod_{j\neq i} (1+|\xi_j|^p)
\end{align*}
for every $\zeta=(0,\dots,0,\zeta_i,0,\dots,0)$ and some $\kappa:(\R^d)^k\to\R_+$ which is locally bounded at the origin.
\end{enumerate}
\todo{There is some inconsistency with $\nu_{n;x}$ and $\nu_{n,x}$. Will try to fix}
\end{theorem}

\begin{proof}
For every $k\in\N$, the sequence $(\nu^k_n)_{n\in\N}\subset\Caratheodory^{k*}([0,T]\times D,U)$ is bounded with norm $\|\nu^k_n\|_{\Caratheodory^{k*}} \equiv 1 < \infty$, and so has a weak*-convergent subsequence. Thus, we can extract a diagonal subsequence $n_j$ such that $\nu^{k}_{n_j} \weaksto \nu^k \in \Caratheodory^{k*}([0,T]\times D, U)$ for every $k\in\N$. For the sake of notational simplicity we denote $n = n_j$. 

We start by showing \textit{(iii)}. Let $\kappa$, $\psi$ and $\phi$ be nonnegative functions, as prescribed. We may assume that $\liminf_{n\to\infty}\int_0^T\psi(t)\Ypair{\nu^k_n}{g}_{\Caratheodory^k}\dd t < \infty$, for otherwise there is nothing to prove. For $M>0$, let $\kappa_M\in C_c(U^k)$, and $\phi_M\in L^1(D^k)$ be the functions $\kappa_M(\xi)=\kappa(\xi)\theta_M(\xi)$ and $\phi_M(x)=\phi(x)\theta_M(x)$. Then $\kappa_M\to\kappa$ and $\phi_M\to\phi$ pointwise almost everywhere as $M\to\infty$. If $g_M(x,\xi):=\phi_M(x)\kappa_M(\xi)$ then clearly $g_M\to g$ as $M\to\infty$ almost everywhere, and $g_M\in \Caratheodory^k(D,U)$ for every $M$. We then find that
\begin{align*}
\int_0^T\psi(t)\Ypair{\nu^k}{g}_{\Caratheodory^k} \dd t&= \lim_{M\to\infty} \int_0^T\psi(t)\Ypair{\nu_t^k}{g_M}_{\Caratheodory^k}\dd t & \text{(Fatou's lemma)}\\
&= \lim_{M\to\infty} \liminf_{n\to\infty}\int_0^T \psi(t) \Ypair{\nu^k_n}{g_M}_{\Caratheodory^k}\dd t & \text{(since $\nu^k_n \weaksto \nu^k$)} \\
&\leq \lim_{M\to\infty} \liminf_{n\to\infty}\int_0^T \psi(t) \Ypair{\nu^k_{t,n}}{g}_{\Caratheodory^k}\dd t & \text{(since $g_M \leq g$ for all $M$)} \\
&= \liminf_{n\to\infty} \int_0^T \psi(t) \Ypair{\nu^k_{t,n}}{g}_{\Caratheodory^k} \dd t,
\end{align*}
which is \eqref{eq:nuklimitbound}.

Since $\nu^k_{n;x,t} \geq 0$ for all $k,n$ and a.e.\ $x,t\in D^k\times[0,T]$, we have $\nu^k_{x,t}\geq0$ for all $k$ and a.e.\ $(x,t)\in D^k\times [0,T]$. To see that $\nu^k_{x,t}(U^k)=1$ for a.e.\ $(x,t)\in D^k\times [0,T]$, let $A_1,\dots,A_k\subset D$ and $B\subset [0,T]$ be bounded Borel sets of positive Lebesgue measure and define $A = A_1\times\dots\times A_k$. Then by \eqref{eq:nuklimitbound},
\begin{equation*}
1 \geq \intavg_B\intavg_A \Ypair{\nu^k_{n;x,t}}{\theta_M}\ dx\ dt \to \intavg_B\intavg_A \Ypair{\nu^k_{x,t}}{\theta_M}\ dx \ dt\qquad \text{as } n\to\infty.
\end{equation*}
Conversely,
\begin{align*}
\intavg_B\intavg|||_A 1-\Ypair{\nu^k_{x,t }}{\theta_M}\ dx\ dt 
&= \lim_{n\to\infty}\intavg_B \intavg_A 1-\Ypair{\nu^k_{n;x,t}}{\theta_M}\ dx\ dt
= \lim_{n\to\infty}\intavg_B \intavg_A \Ypair{\nu^k_{n;x,t}}{1-\theta_M}\ dx \ dt\\
&\leq \limsup_{n\to\infty} \frac{1}{M^p}\intavg_B \intavg_A \Ypair{\nu^k_{n;x,t}}{|\xi|^p}\ dx\ dt \\
&= \limsup_{n\to\infty} \frac{1}{M^p} \sum_{i=1}^k\intavg_B \intavg_A\Ypair{\nu^k_{n;x,t}}{|\xi_i|^p}\ dx \ dt \\
&\leq \frac{1}{M^p}\sum_{i=1}^k\frac{c^p}{|A_i||B|},
\end{align*}
where we have first used Chebysheff's inequality and then the uniform $L^p$ bound \eqref{eq:uniformlpbound}. Passing to $M\to\infty$ in the two estimates above shows that
\begin{equation}\label{eq:numassone}	% nu has mass 1
\intavg_B\intavg_A \nu^k_{x}(U^k)\ dx\ dt = 1.
\end{equation}
Since $A_1,\dots,A_k$ and $B$ were arbitrary, it follows that $\nu^k_{x,t}(U^k) = 1$ for a.e.\ $x,t\in D^k\times[0,T]$.


The limit $\cm$ clearly satisfies the symmetry condition. 
%For consistency, let $f\in C_0(U^{k-1})$ and $A_1,\dots,A_k\subset D$ be bounded and measurable, and let $A = A_1\times\cdots\times A_k$. It is evident that consistency will follow provided
%\[
%\int_{A}\int_{U^k} f(\xi_1,\dots,\xi_{k-1})\,d\nu^k_{x_1,\dots,x_k}\,dx = \int_{A} \int_{U^{k-1}} f(\xi_1,\dots,\xi_{k-1})\,d\nu^{k-1}_{x_1,\dots,x_{k-1}}\,dx,
%\]
%irrespective of $A_1,\dots,A_k$ and $f$. Moreover, we can assume that $f \geq 0$. Letting $\phi(x) = \ind_A(x)$ and $\kappa(\xi_1,\dots,\xi_k) = f(\xi_1,\dots,\xi_{k-1})$ in \eqref{eq:nuklimitbound} then gives
%\begin{align*}
%\int_{A}\int_{U^k} f(\xi_1,\dots,\xi_{k-1})\,d\nu^k_{x_1,\dots,x_k}\,dx 
%&\leq \liminf_n \int_{A}\int_{U^k} f(\xi_1,\dots,\xi_{k-1})\,d\nu^k_{n;x_1,\dots,x_k}\,dx \\
%&= \liminf_n \int_{A}\int_{U^{k-1}} f(\xi_1,\dots,\xi_{k-1})\,d\nu^{k-1}_{n;x_1,\dots,x_{k-1}}\,dx \\
%&= \int_{A}\int_{U^{k-1}} f(\xi_1,\dots,\xi_{k-1})\,d\nu^{k-1}_{x_1,\dots,x_{k-1}}\,dx
%\end{align*}
For consistency, we need to show that for any $f\in C_0(U^{k-1})$ and $\phi\in C_c(D^k)$, we have
\begin{equation}\label{eq:symmetry}
\int_{D^k} \phi(x)\Ypair{\nu^k_{x,t}}{f(\xi_1,\dots,\xi_{k-1})}\ dx = \int_{D^k} \phi(x)\Ypair{\nu^{k-1}_{x_1,\dots,x_{k-1},t}}{f(\xi_1,\dots,\xi_{k-1})}\ dx,
\end{equation}
for almost all $t\in[0,T]$. To this end, we will show that
\begin{equation}
\label{eq:time_symmetry}
\int_0^T\psi(t)\int_{D^k} \phi(x)\Ypair{\nu^k_{x,t}}{f(\xi_1,\dots,\xi_{k-1})}\ dx \ dt= \int_0^T\psi(t)\int_{D^k} \phi(x)\Ypair{\nu^{k-1}_{x_1,\dots,x_{k-1},t}}{f(\xi_1,\dots,\xi_{k-1})}\ dx \ dt,
\end{equation}
for every $\psi\in C([0,T])$.
\todo[inline]{KOL: This can probably be done without integrating over $t$, but it makes the argument slightly cleaner, in my opinon.}

Define $\bar{f}_M\in C_0(U^k)$ by $\bar{f}_M(\xi_1,\dots,\xi_k) = f(\xi_1,\dots,\xi_{k-1})\theta_M(\xi_k).$ We estimate the difference between the left- and right-hand sides of \eqref{eq:time_symmetry} by $E_1+E_2+E_3+E_4$, where
\begin{align*}
E_1 &= \left|\int_0^T\psi(t)\int_{D^k}\phi(x)\Ypair{\nu^k_{x,t}}{f(\xi_1,\dots,\xi_{k-1})-\bar{f}_M(\xi)}\ dx\ dt\right| \\
E_2 &= \left|\int_0^T\psi(t) \int_{D^k}\phi(x)\left(\Ypair{\nu^k_{x,t}}{\bar{f}_M(\xi)} - \Ypair{\nu^k_{n;x,t}}{\bar{f}_M}\right)\ dx\ dt\right| \\
E_3 &= \left|\int_0^T\psi(t) \int_{D^k}\phi(x)\left(\Ypair{\nu^k_{n;x,t}}{\bar{f}_M} - \Ypair{\nu^{k-1}_{n;\hat{x}_k,t}}{f}\right)\ dx\ dt\right| \\
E_4 &= \left|\int_0^T\psi(t)\int_{D^k}\phi(x)\left(\Ypair{\nu^{k-1}_{n;\hat{x}_k,t}}{f} - \Ypair{\nu^{k-1}_{\hat{x}_k,t}}{f}\right)\ dx\ dt\right|
\end{align*}
where $\hat{x}_k = (x_1,\dots,x_{k-1})$. 
The fact that $E_1\to0$ as $M\to\infty$ follows from the Dominated Convergence Theorem. For every $M>0$ we have $E_2$, $E_4 \to 0$ as $n\to\infty$ by the weak* convergence of $\nu^k_n$ and $\nu^{k-1}_n$, respectively. For $E_3$ we can write
\begin{align*}
E_3 &= \left|\int_0^T\psi(t) \int_{D^k}\phi(x)\Ypair{\nu^k_{n;x,t}}{f\bigl(\xi_1,\dots,\xi_{k-1}\bigr)\bigl(\theta_M(\xi_k)-1\bigr)}\ dx\ dt\right| \\
&\leq \|f\|_{C_0(U^{k-1})}\|\phi\|_{C_0(D^k)}\|\psi\|_{C([0,T])}\int_{\supp(\psi)}\psi(t)\int_{\supp(\phi)}\Ypair{\nu^1_{n;x_k}}{1-\theta_M(\xi)}\ dx \ dt\\
&\leq \|f\|_{C_0(U^{k-1})}\|\phi\|_{C_0(D^k)}\|\psi\|_{C([0,T])}\frac{C}{M^p} \to 0
\end{align*}
as $M\to\infty$ (as in the proof of \eqref{eq:numassone}). Thus, for a given $\eps>0$ we can first select $M$ such that $E_1,E_3<\eps$, and then select $n$ such that $E_2,E_4<\eps$. This proves \eqref{eq:time_symmetry}, which again proves \eqref{eq:symmetry} for almost all $t\in[0,T]$.

The $L^p$ bound \textit{(i)} follows from \eqref{eq:nuklimitbound} with $k=1$, $\phi\equiv 1$, $\psi\equiv 1$ and $\kappa(\xi) = |\xi|^p$, since $\Ypair{\nu^1}{|\xi|^p}_{\Caratheodory^1} \leq \liminf_n \Ypair{\nu^1_n}{|\xi|^p}_{\Caratheodory^1} \leq c^p$, by \eqref{eq:uniformlpbound}. To prove the diagonal continuity of $\cm$ we use \eqref{eq:nuklimitbound} with $k=2$, $\phi(x,y) = \frac{\Indicator{B_r(x)}(y)}{|B_r(x)|}$, $\kappa(\xi_1,\xi_2) = |\xi_1-\xi_2|^p$ and $\psi\in L^1([0,T])\cap L^\infty([0,T])$ arbitrary,  and note that $\omega_r^p(\nu_t^2) = \Ypair{\nu^2_t}{g}_{\Caratheodory^2}^p$. The DC of $\nu^2_t$ for almost all $t\in[0,T]$ then follows from $\int_0^T\psi(t)\omega_r^p(\nu^2_t)\ dt \leq \liminf_{n\to\infty}\int_0^T \psi(t) \omega_r^p(\nu^2_{n;t})\ dt \to 0$ as $r\to0$, by \eqref{eq:uniformdc}.

We prove \textit{(iv)} for $k=1$ and give a sketch of the general case. Let $\psi\in L^1([0,T])$, and let $g$ be a Carath\'eodory function such that $|g(x,\xi)|\leq C_g(1+|\xi|^p)$ for some $C_g>0$ and $|g(x,\xi)-g(y,\zeta)| \leq \kappa(x-y)\max(|\xi|,|\zeta|)^{p-1}|\xi-\zeta|$ for some $\kappa:\R^{d}\to\R_+$ which is locally bounded at the origin. By approximating $g$ by a function with bounded support, we may assume that $D$ is bounded. Define
\begin{align*}
u_n(x) := \int_0^T\psi(t)\Ypair{\nu^1_{n;x,t}}{g(x,\xi)}\ dt, && u_n^M(x) := \int_0^T\psi(t)\Ypair{\nu^1_{n;x,t}}{\theta_M(|\xi|^p)g(x,\xi)}\ dt, \\
u(x) := \int_0^T\psi(t)\Ypair{\nu^1_{x,t}}{g(x,\xi)}\ dt, && u^M(x) := \int_0^T\psi(t)\Ypair{\nu^1_{x,t}}{\theta_M(|\xi|^p)g(x,\xi)}\ dt.
\end{align*}
The sequence $\{u_n\}_n$ satisfies
\begin{equation}\label{eq:udiagcontargument}
\begin{split}
\int_D\intavg_{B_r(0)} &|u_n(x+z)-u_n(x)|\,dzdx \leq \int_0^T|\psi(t)|\int_D\intavg_{B_r(0)}\big|\Ypair{\nu^2_{n,x,x+z,t}}{g(x+z,\xi_2)-g(x,\xi_1)}\big|\,dzdxdt \\
&\leq \int_0^T|\psi(t)|\int_D\intavg_{B_r(0)}\Ypair{\nu^2_{n,x,x+z,t}}{\kappa(|z|)\max(|\xi_1|,|\xi_2|)^{p-1}|\xi_2-\xi_1|}\,dz dx dt\\
&\leq 
\|\psi\|_{L^\infty([0,T])}\|\kappa\|_{L^\infty(B_r(0))}\left(\int_0^T\int_D\intavg_{B_r(0)}\Ypair{\nu^2_{n,x,x+z,t}}{\max(|\xi_1|,|\xi_2|)^p}\,dz dx dt\right)^{(p-1)/p} \\
&\qquad \qquad \qquad\quad \left( \int_0^T\int_D\intavg_{B_r(0)}\Ypair{\nu^2_{n,x,x+z,t}}{|\xi_2-\xi_1|^p}\,dz dx dt\right)^{1/p} \\
&\leq 2\|\psi\|_{L^\infty([0,T])}\|\kappa\|_{L^\infty(B_r(0))}c^{p-1} \int_0^T\omega_r^p(\nu^2_{n,t})\ dt,
\end{split}
\end{equation}
so together with the uniform bound $\|u_n\|_{L^1(D)} \leq C_g(|D|+c)$ we can apply Kolmogorov's Compactness Theorem \cite[Theorem A.5]{HR} to conclude that $\{u_n\}_{n\in\N}$ is precompact in $L^1(D)$. Hence, there exists a subsequence $u_{n_l}$ and some $\bar{u}\in L^1(D)$ such that $u_{n_l}\to\bar{u}$ as $l\to\infty$ in $L^1(D)$. From the weak* convergence of $\nu^1_n$ we know that $u_n^M \weakto u^M$ as $n\to\infty$ weakly in $L^1(D)$ for every $M>0$. Lebesgue's dominated convergence theorem implies that $u^M \to u$ as $M\to\infty$ in $L^1(D)$. 
%Last, by the Dunford--Pettis theorem, the precompactness of $\{u_n\}_{n\in\N}$ implies the uniform integrability property
%\[
%\lim_{M\to\infty}\sup_{n\in\N}\int_D |u_n(x)| \Indicator{[M,\infty]}(|u_n(x)|)\,dx = 0
%\]

We claim that $u^M_n \to u_n$ as $M\to\infty$ in $L^1(D)$, \textit{uniformly} in $n$. Indeed, choosing $r>0$ such that $M\geq \frac{1}{|B_r|^{1/p}}C$ (where $C$ is the constant in \eqref{eq:LpLinftybound}), we get
\todo{Here we probably want to change the assumption of diagonal continuity.}
\begin{align*}
\int_D |u_n(x)-u_n^M(x)|\,dx &= \int_D \big|\int_0^T\psi(t)\Ypair{\nu^1_{n;x,t}}{(1-\theta_M(|\xi|^p))g(x,\xi)}\ dt \big|\,dx \\
&\leq C_g\int_D \int_0^T\psi(t)\Ypair{\nu^1_{n;x,t}}{\big||\xi|^p-\theta_M(|\xi|^p)|\xi|^p\big|}\,dt dx \\
&= C_g\int_0^T\psi(t)\int_{L^p(D)}\int_D \big||u(x)|^p - \zeta_M(|u(x)|^p)\big|\,dxd\mu_n(u) dt\\
&\leq 3C_g\int_0^T\psi(t)\int_{L^p(D)} \omega_r^p(u)^p\,d\mu_{n,t}(u)\ dt \\
&= 3C_g\|\psi\|_{L^\infty([0,T])}\int_0^T\omega_r^p(\nu^2_{n,t})^p\ dt
\end{align*}
where the last inequality follows from Lemma \ref{lem:cutoff} together with the $L^p$ bound \eqref{eq:LpLinftybound}. The final term above vanishes as $M\to\infty$ uniformly in $n$, by the uniform diagonal continuity assumption \eqref{eq:uniformdc}. It follows that for any $\phi\in L^\infty(D)$,
\begin{align*}
\Big|\int_D \phi(u-\bar{u})\,dx\Big| &\leq \|\phi\|_{L^\infty}\Big(\|u-u^M\|_{L^1}+\|u_{n_l}^M-u_{n_l}\|_{L^1} + \|u_{n_l}-\bar{u}\|_{L^1}\Big) + \Big|\int_D \phi\big(u^M-u_{n_l}^M\big)\,dx\Big|,
\end{align*}
all of which vanish as $M\to\infty$ and $l\to\infty$. We conclude that $\bar{u}=u$, whence $u_{n_l}\to u$ as $l\to\infty$. By the uniqueness of the limit we get convergence of the whole sequence: $u_n \to u$ in $L^1(D)$ as $n\to\infty$.

For general $k\in\N$ we prove only that $u_n(x):=\Ypair{\nu^k_{n;x,t}}{g(x,\xi)}$ satisfies a bound of the form \eqref{eq:udiagcontargument}, and leave the rest to the reader. As above we may assume that $D$ is bounded. We write first
\begin{align*}
&\int_{D^k}\intavg_{B_r(0)^k}|u_n(x+z)-u_n(x)|\,dzdx \\
&\leq \int_{D^k}\intavg_{B_r(0)^k}\int_0^T|\psi(t)|\Ypair{\nu^{2k}_{n;x,x+z,t}}{\big|g\big(x+z,\xi_{k+1},\dots,\xi_{2k}\big)-g\big(x,\xi_1,\dots,\xi_k\big)\big|}\,dtdzdx \\
&\leq \sum_{l=1}^k \int_{D^k}\intavg_{B_r(0)^k}\int_0^T|\psi(t)|\kappa(z)\Ypair{\nu^{2k}_{n;x,x+z,t}}{|\xi_{l+k}-\xi_l|\max(|\xi_l|,|\xi_{l+k}|)^{p-1}{\textstyle\prod_{i\neq l}}(1+|\xi_i|^p)}\,dzdxdt  \\
&\leq \|\psi\|_{L^\infty([0,T])}\|\kappa\|_{L^\infty(B_r(0)^k)}\sum_{l=1}^k \int_0^T\int_{D^k}\intavg_{B_r(0)^k}\Ypair{\nu^{2k}_{n;x,x+z,t}}{|\xi_{l+k}-\xi_l|\max(|\xi_l|,|\xi_{l+k}|)^{p-1}{\textstyle\prod_{i\neq l}}(1+|\xi_i|^p)}\,dzdxdt.
\end{align*}
Consider, say, the last summand above:
\begin{align*}
\int_0^T\int_{D^k}&\intavg_{B_r(0)^k}\Ypair{\nu^{2k}_{n;x,x+z,t}}{|\xi_{2k}-\xi_k|\max(|\xi_k|,|\xi_{2k}|)^{p-1}{\textstyle\prod_{i=1}^{k-1}}(1+|\xi_i|^p)}\,dzdxdt \\
&=\int_0^T\int_{D^k}\intavg_{B_r(0)}\Ypair{\nu^{k+1}_{n;x,x_k+z_k,t}}{|\xi_{k+1}-\xi_k|\max(|\xi_k|,|\xi_{k+1}|)^{p-1}{\textstyle\prod_{i=1}^{k-1}}(1+|\xi_i|^p)}\,dz_kdxdt \\
&=\int_0^T\int_{L^p(D)}\int_{D^k}\intavg_{B_r(0)}\big|u(x_k+z_k)-u(x_k)\big|\max(|u(x_k)|,|u(x_k+z_k)|)^{p-1}\\
&\qquad\qquad\qquad\qquad\quad \prod_{i=1}^{k-1}\big(1+|u(x_i)|^p\big)\,dz_kdxd\mu_{n,t}(u)dt \\
&=\int_{L^p(D)}\left(\int_{D}\intavg_{B_r(0)}|u(x_k+z_k)-u(x_k)|\max(|u(x_k)|,|u(x_k+z_k)|)^{p-1}\,dz_kdx_k\right) \\
&\qquad\qquad\quad\prod_{i=1}^{k-1}\left(\int_D 1+|u(x_i)|^p\,dx_i\right)\,d\mu_{n,t}(u) \\
&\leq 2\int_0^T\int_{L^p(D)}\left(\int_{D}\intavg_{B_r(0)}|u(x_k+z_k)-u(x_k)|^p\,dz_kdx_k\right)^{1/p}\left(\int_D |u(x_k)|^p\,dx_k\right)^{1-1/p} \\
&\qquad\qquad\quad \prod_{i=1}^{k-1}\left(\int_D 1+|u(x_i)|^p\,dx_i\right)\,d\mu_{n,t}(u)dt \\
&\leq 2\int_0^T\omega_r^p(\nu^2_{n,t})\ dt C^{1-1/p}\big(|D|+C^p\big)^{k-1}
\end{align*}
where the last inequality follows from \eqref{eq:LpLinftybound}. By the boundedness of $D$ and the uniform diagonal continuity of $\cm_n$, the above vanishes uniformly as $r\to0$. The rest of the proof follows as in the proof for $\nu^1$.
\end{proof}




\subsection{Statistical solutions}\label{sec:statsoln}
Using correlation measures we can now define statistical solutions of \eqref{eq:cl}. Statistical solutions are correlation measures---or equivalently, probability measures over $L^1$---that satisfy the differential equation \eqref{eq:cl} in a certain averaged sense. The full derivation can be found in \cite{FLM17}, and we provide the rigorous definition below.
\begin{definition}\label{def:statsoln}
Let $\bar{\mu}\in\Prm\big(L^1\big(\R^d,\R^N\big)\big)$ have bounded support,
\begin{equation}\label{eq:fastdecay}
\|u\|_{L^1(\R^d,\R^N)} \leq C \qquad \text{for $\bar{\mu}$-a.e. } u\in L^1(\R^d,\R^N)
\end{equation}
for some $C>0$. A \emph{statistical solution} of \eqref{eq:cl} with initial data $\bar{\mu}$ is a weak*-measurable mapping $t \mapsto \mu_t\in \Prm\big(L^1\big(\R^d,\R^N\big)\big)$ such that each $\mu_t$ has bounded support, and such that the corresponding correlation measures $(\nu^k_t)_{k\in\N}$ satisfy 
\begin{equation}\label{eq:momentcorrmeas}
\partial_t \Ypair{\nu^k_{t,x}}{\xi_1\otimes\cdots\otimes\xi_k} + \sum_{i=1}^k \nabla_{x_i}\cdot\Ypair{\nu^k_{t,x}}{\xi_1\otimes\cdots\otimes f(\xi_i)\otimes\cdots\otimes\xi_k} = 0
\end{equation}
in the sense of distributions, i.e.
\begin{gather*}
\int_{\R_+}\int_{(\R^d)^k} \Ypair{\nu^k_{t,x}}{\xi_1\otimes\cdots\otimes\xi_k}:\partial_t \phi + \sum_{i=1}^k \Ypair{\nu^k_{t,x}}{\xi_1\otimes\cdots\otimes f(\xi_i)\otimes\cdots\otimes\xi_k}: \nabla_{x_i}\phi\,dxdt \\
+ \int_{(\R^d)^k}\Ypair{\bar{\nu}^k_x}{\xi_1\otimes\cdots\otimes\xi_k}\phi\bigr|_{t=0}\,dx = 0
\end{gather*}
for every $\phi\in C_c^\infty\Big(\big(\R^d\big)^k\times\R_+,\ \big(\R^N\big)^{\otimes k}\Big)$ and for every $k\in\N$. (Here, $\bar{\cm}$ denotes the correlation measure associated with the initial probability measure $\bar{\mu}$.)
\end{definition}
